Applied metamodelling for ATM performance simulations

The use of Air traffic management (ATM) simulators for planing and operations can be challenging due to their modelling complexity. This paper presents XALM (eXplainable Active Learning Metamodel), a three-step framework integrating active learning and SHAP (SHapley Additive exPlanations) values into simulation metamodels for supporting ATM decision-making. XALM efficiently uncovers hidden relationships among input and output variables in ATM simulators, those usually of interest in policy analysis. Our experiments show XALM's predictive performance comparable to the XGBoost metamodel with fewer simulations. Additionally, XALM exhibits superior explanatory capabilities compared to non-active learning metamodels. Using the `Mercury' (flight and passenger) ATM simulator, XALM is applied to a real-world scenario in Paris Charles de Gaulle airport, extending an arrival manager's range and scope by analysing six variables. This case study illustrates XALM's effectiveness in enhancing simulation interpretability and understanding variable interactions. By addressing computational challenges and improving explainability, XALM complements traditional simulation-based analyses. Lastly, we discuss two practical approaches for reducing the computational burden of the metamodelling further: we introduce a stopping criterion for active learning based on the inherent uncertainty of the metamodel, and we show how the simulations used for the metamodel can be reused across key performance indicators, thus decreasing the overall number of simulations needed.

==> table_with_hotspotsolver.tex <==
\begin{table}[!ht]
    \centering
    \caption{Performance of the metamodels. The standard deviation is given in parentheses.}
    \label{tab:performance}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lrrrrl}
    \toprule
    & \textbf{\#sim} & \textbf{RMSE} & \textbf{RRSE} &\textbf{Correlation}& \textbf{Hyperparameters}\\ 
    \midrule
    {\textbf{Flight arrival delay}}  &      &      \\
    Mean predictor        &50000&   106.0   &  1.00  & - &-  \\
    XGBoost         & 50000        &   3.90   &  0.04  & 1.0 & Max depth = 3, learning rate = 0.01, L2-reg. = 0.5 \\
    GP & 1000  &  4.01 &  0.04 &  1.0 & - \\
    GP & 100  &  4.45 (0.26) &  0.04 (0.00) &  1.0 (0.00) & - \\
    GP & 30  &   5.68 (0.57) &  0.05 (0.01) &  1.0 (0.00) & - \\ 
    %GP (multiple KPIs) & 30  &  ?    & ?  & - \\
    \midrule
    {\textbf{Flight departure delay}}  &      &      \\
    Mean predictor        &50000&   106.4   &  1.00  & - & -  \\
    XGBoost         & 50000        &   3.86   &  0.04  & 1.0 & Max depth = 3, learning rate = 0.01, L2-reg. = 0.5 \\
    GP & 1000 & 3.93 & 0.04 & 1.0 & - \\
    GP & 100  &  4.34 (0.22) &  0.04 (0.00) &  1.0 (0.00) & - \\ 
    GP & 30  &   5.44 (0.56) &  0.05 (0.01) &  1.0 (0.00) & - \\
    %GP (multiple KPIs) & 30  &  ?    & ?  & - \\
    \midrule
    {\textbf{Passenger arrival delay}}\\
    Mean predictor        &50000& 202.3     &   1.00  & - & - \\
    XGBoost         & 50000        &  43.0    &    0.21  & .98& Max depth = 5, learning rate = 0.05, L2-reg. = 0.4 \\ 
    GP & 1000 & 43.9 & 0.22 & .98 & - \\
    GP & 100  &   48.0 (2.23) &  0.24 (0.01) &  .97 (0.00) & - \\
    GP & 30  &   56.6 (4.96) &  0.28 (0.02) &  .96 (0.01) & - \\
    %GP (multiple KPIs) & 30  &  ?    & ?  & - \\
    \midrule
    {\textbf{Planned absorbed delay}}  &      &      \\
    Mean predictor        &50000&   0.242   &  1.00  & - & -  \\
    XGBoost         & 50000        &   0.094   &  0.39  & .92 & Max depth = 3, learning rate = 0.10, L2-reg. = 0.5 \\
    GP & 1000 & 0.10 & 0.41 & 91 & -\\
    GP & 100  & 0.106 (0.004) &  0.44 (0.02) &  .90 (0.01) & - \\
    GP & 30  &   0.134 (0.016) &  0.55 (0.07) &  .86 (0.03) & - \\
    %GP (multiple KPIs) & 30  &  ?    & ?  & - \\
    \midrule
    {\textbf{Holding time}}  &      &      \\
    Mean predictor        &50000&   0.204   &  1.00  & - & -  \\
    XGBoost         & 50000        &   0.160   &  0.78 & .62 & Max depth = 3, learning rate = 0.20, L2-reg. = 0.5 \\
    GP & 1000 & 0.163 & 0.80 & .60 & - \\
    GP & 100  &  0.179 (0.012) &  0.88 (0.06) &  .54 (0.05) & - \\
    GP & 30  &   0.213 (0.024) &  1.05 (0.12) &  .42 (0.10) & - \\
    %GP (multiple KPIs) & 30  &  ?    & ?  & - \\
    \midrule
    {\textbf{Fuel cost}}  &      &      \\
    Mean predictor        &50000&   26401   &  1.00  & - & -  \\
    XGBoost         & 50000        &   345   &  0.01  & 1.0 & Max depth = 4, learning rate = 0.01, L2-reg. = 0.4 \\
    GP & 1000 & 362 & 0.01 & 1.0 & - \\
    GP & 100  &  411 (20.3) &  0.02 (0.00) &  1.0 (0.00) & - \\
    GP & 30  &   534 (56.8) &  0.02 (0.00) &  1.0 (0.00) & - \\
    %GP (multiple KPIs) & 30  &  ?    & ?  & - \\
    \bottomrule
    \end{tabular}
    }
\end{table}







% Table with active learning performance for GP 30 and 100 (w/o HS)
\begin{table}[!ht]
    \centering
    \caption{Performance of the metamodels. The standard deviation is given in parentheses. The time is computed as the sum of the simulation time (2.5 minutes per simulation) and the fitting time for the algorithm (incl. the active learning for the GP with 30 and 100 simulations).} 
    \label{tab:performance}
    %\resizebox{\textwidth}{!}{
    \begin{tabular}{llrrrrl}
    \toprule
    \textbf{KPI} & \textbf{Model} & \textbf{\#sim} & \textbf{RMSE} & \textbf{RRSE} &\textbf{Correlation}\\%& \textbf{Time [hr]} \\ 
    \midrule
    {\textbf{Flight arrival delay}}  &
    Mean predictor        &50000&   106.0   &  1.00  & - \\%&2083.33\\
    & XGboost         & 50000        &   3.91 (0.00)   &  0.04 (0.00) & 1.0 (0.00) \\%& 2083.34 \\
    & XGboost         & 1000        &   4.27 (0.04)   &  0.04 (0.00) & 1.0 (0.00)\\% & 41.67 \\
    & GP & 1000  &  3.97 (0.01) &  0.04 (0.00) &  1.0 (0.00) \\%& 41.83\\
    & GP & 100  &  4.22 (0.08) &  0.04 (0.00) &  1.0 (0.00) \\%&  4.9 \\ 
    & GP & 30  &   5.24 (0.29) &  0.05 (0.00) &  1.0 (0.00) \\%&  1.4 \\ 
    %{\color{red}GP} (multiple KPIs) & 30  &  ?    & ? \\
    \midrule
    {\textbf{Flight departure delay}}  &
    Mean predictor        &50000&   106.4   &  1.00  & - \\%&2083.33 \\
    & XGboost         & 50000        &   3.86 (0.00)   &  0.04 (0.00)  & 1.0 (0.00) \\%& 2083.34 \\
    & XGboost         & 1000        &   4.23 (0.04)   &  0.04 (0.00)  & 1.0 (0.00) \\%& 41.67 \\
    & GP & 1000 & 3.90 (0.01) & 0.04 (0.00) & 1.0 (0.00) \\%& 41.83\\
    & GP & 100  &  4.13 (0.09) &  0.04 (0.00) &  1.0 (0.00) \\%&  4.9 \\  
    & GP & 30  &   5.17 (0.41) &  0.05 (0.00) &  1.0 (0.00) \\%&  1.39 \\ 
    %{\color{red}GP} (multiple KPIs) & 30  &  ?    & ? \\
    \midrule
    {\textbf{Passenger arrival delay}} & 
    Mean predictor        &50000& 202.3     &   1.00  & - \\%& 2083.33\\
    & XGboost         & 50000        &  43.0 (0.03)   &    0.21 (0.00)  & .98 (0.00) \\%& 2083.34 \\
    & XGboost         & 1000        &  46.2 (0.46)   &    0.23 (0.00)  & .97 (0.00) \\%& 41.67  \\
    & GP & 1000 & 43.7 (0.17) & 0.22 (0.00) & .98 (0.00) \\%& 41.83\\
    & GP & 100  &   47.2 (1.37) &  0.23 (0.01) &  .97 (0.00) \\%&  4.9 \\
    & GP & 30  &   54.1 (6.01) &  0.27 (0.03) &  .97 (0.01) \\%&  1.4 \\
    %{\color{red}GP} (multiple KPIs) & 30  &  ?    & ? \\
    \midrule
    {\textbf{Planned absorbed delay}}  & 
    Mean predictor        &50000&   0.242   &  1.00  & - \\%& 2083.33 \\
    & XGboost         & 50000        &   0.093 (0.000)   &  0.39 (0.00)  & .92 (0.00) \\%& 2083.33 \\
    & XGboost         & 1000        &   0.098 (0.001)   &  0.41 (0.00)  & .92 (0.00) \\%& 41.67   \\
    & GP & 1000 & 0.100 (0.001) & 0.41 (0.00) & 92 (0.00) \\%& 41.82 \\
    & GP & 100  & 0.106 (0.004) &  0.44 (0.02) &  .91 (0.00) \\%&  4.92 \\ 
    & GP & 30  &   0.120 (0.010) &  0.50 (0.04) &  .88 (0.02) \\%&  1.42 \\ 
    %{\color{red}GP} (multiple KPIs) & 30  &  ?    & ? \\
    \midrule
    {\textbf{Holding time}}  &      
    Mean predictor        &50000&   0.204   &  1.00  & - \\%&2083.33 \\
    & XGboost         & 50000        &   0.160 (0.000)   &  0.78 (0.00) & .62 (0.00) \\%& 2083.33\\
    & XGboost         & 1000        &   0.166 (0.002)   &  0.81 (0.01) & .59  (0.01) \\%& 41.67 \\
    & GP & 1000 & 0.163 (0.001) & 0.80 (0.00) & .60 (0.00) \\%& 41.82\\
    & GP & 100  &  0.171 (0.004) &  0.84 (0.02) &  .57 (0.02) \\%&  5.05 \\
    & GP & 30  &   0.197 (0.021) &  0.96 (0.10) &  .46 (0.11) \\%&  1.53 \\
    %{\color{red}GP} (multiple KPIs) & 30  &  ?    & ? \\
    \midrule
    {\textbf{Fuel cost}}  &      
    Mean predictor        &50000&   26401   &  1.00  & - \\%&2083.33 \\
    & XGboost         & 50000        &   354 \phantom{0}(0.4)   &  0.01 (0.00)  & 1.0 (0.00) \\%& 2083.34 \\
    & XGboost         & 1000        &   474 (10.6)   &  0.02 (0.00)  & 1.0 (0.00) \\%& 41.67 \\
    & GP & 1000 & 362 \phantom{0}(2.6) & 0.01 (0.00) & 1.0 (0.00)\\% & 41.92 \\
    & GP & 100  &  391 (14.3) &  0.01 (0.00) &  1.0 (0.00) \\%&  18.51  \\ 
    & GP & 30  &   468 (48.9) &  0.02 (0.00) &  1.0 (0.00) \\% &  3.05  \\
    %{\color{red}GP} (multiple KPIs) & 30  &  ?    & ? \\
    \bottomrule
    \end{tabular}
    %}
\end{table}
